IoT Device Labeling Using Large Language Models

The IoT market is diverse and characterized by a multitude of vendors that support different device functions (e.g., speaker, camera, vacuum cleaner, etc.). Within this market, IoT security and observability systems use real-time identification techniques to manage these devices effectively. Most existing IoT identification solutions employ machine learning techniques that assume the IoT device, labeled by both its vendor and function, was observed during their training phase. We tackle a key challenge in IoT labeling: how can an AI solution label an IoT device that has never been seen before and whose label is unknown? Our solution extracts textual features such as domain names and hostnames from network traffic, and then enriches these features using Google search data alongside catalog of vendors and device functions. The solution also integrates an auto-update mechanism that uses Large Language Models (LLMs) to update these catalogs with emerging device types. Based on the information gathered, the device's vendor is identified through string matching with the enriched features. The function is then deduced by LLMs and zero-shot classification from a predefined catalog of IoT functions. In an evaluation of our solution on 97 unique IoT devices, our function labeling approach achieved HIT1 and HIT2 scores of 0.7 and 0.77, respectively. As far as we know, this is the first research to tackle AI-automated IoT labeling.

==> Features.tex <==
\section{Features}
\label{sec:features_and_enrichment}
Our approach is based on obtaining textual features from the traffic logs of a device. Formally, we use the \emph{Feature Type} set of size 5, as follows: 

\begin{definition}
Let $FT$  be the Feature Type  set of \{hostname, domains, Transport Layer Security (TLS) Issuer, Organizationally Unique Identifier (OUI), UserAgent \} \\
\end{definition}

Table \ref{tbl:features} %(see Appendix B) \barm{I'm not sure how interesting this is... Anat, should i move it into the paper?}
presents the feature types, the protocol from which they originate,   their possible encryption, and their availability in the LAN or WAN\footnote{ The LAN information can also be retrieved using the TR69 protocol from the router.}. The Domain feature, obtained from the DNS protocol, typically lacks encryption since  DoH \cite{rfc7858} and DoT \cite{rfc8484} are not commonly used in IoT due to the limited processing power of IoT devices. The TLS Issuer feature, derived from the TLS protocol, is available because it is exchanged before encryption commences. 
\begin{table}[b!]
\centering

\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l||c|c|c|}
\hline
\textbf{Feature} & \textbf{Protocol} & \textbf{Encryption} & \textbf{Availability}\\
\hline
\hline
Domains & DNS & Not common & LAN and WAN \\
\hline
Hostname & DHCP & No encryption & LAN \\
\hline
TLS Issuer & TLS & No encryption & LAN and WAN \\
\hline
User Agent & HTTP & Encrypted in https & LAN and WAN \\
\hline
OUI & MAC & No encryption & LAN \\
\hline
\end{tabular}
}
\caption{Feature types and their properites: protocol, encryption and observability in the network (LAN or WAN)}
\label{tbl:features}

\end{table}

Because different feature types have different numbers of values, we define the feature values of a feature type $t$ as a vector, according to the following.
\begin{definition}
  Let $f_t$ be the vector of feature values of $t\in FT$. Where $f_{t} = (f_{t,1}...f_{t,m})$ , and   
  $f_{t,k}$ is the  $kth$ feature value (where $m<|f_t|$).
  \newline
\end{definition}

Table \ref{tab:avg_sv_fields_unique}  presents the average and standard deviation of the feature values, although hostname is available only in 60\% of the devices. Devices may lack features for various reasons. The absence of specific traffic types like HTTP or TLS can lead to a situation with no User-Agents and no TLS-Issuer. Moreover, short traffic logs can omit features, such as missing hostnames due to uncaptured DHCP messages \cite{rfc2131}. 
Our labeling algorithm  works with the inherent variation in the quantity of feature values. 


\ignore{ but seems to be stable across different datasets, as observed in Figure \ref{fig:availability_and_accuacy_features}.}


\begin{table}[ht]
\centering
%\resizebox{\columnwidth}{!}{%
\begin{tabular}{lc}
\toprule
Feature & Average Number of values $\pm$ SV \\
\midrule
Hostname & 0.68 $\pm$ 0.51 \\
Domains & 20.36 $\pm$ 37.02 \\
User-agents & 4.98 $\pm$ 12.98 \\
TLS Issuer & 1.74 $\pm$ 3.00 \\
OUI & 0.97 $\pm$ 0.17 \\
\bottomrule
\end{tabular}
%}
\caption{The average number of values and the associated standard deviation for each feature type.}
\label{tab:avg_sv_fields_unique}

\end{table}


==> List.tex <==
\subsection{Explainability}
Explainability in AI models is essential, especially when the system is required to supply the users a clear understanding of how decisions are made regarding the IoT device labels. 
%A model's ability to provide insight into its reasoning not only boosts user confidence but also enables potential debugging and refinement of the model. 



We provide here  a few examples of results that enable the user to decide whether the model labeled a device correctly or not. The basic approach is to print to the user the top enriched featured with the highest score that maps to the chosen label. 


\begin{mdframed}[frametitle={Search results from a blog post named "Capturing the Connections: Unboxing Internet of Things"\cite{203628}. Device Vendor: WeMo, Device Function: Plug.}]
'After each on/off event the WeMo contacts api.xbcs.net using an encrypted communication. When the user plugs the light bar into the WeMo an encrypted...'
\end{mdframed}

\begin{mdframed}[frametitle={Search results the Hostname 
"MyQ-139"\cite{myq_hostname_blog}.\newline
Device Vendor: MYQ, Device Function: Garage Door}]
{'... it working in 2.0 also. Does anyone know if the API yet allows us to control the garage door ...'}
\end{mdframed}

\subsection{Vendors and Type Catalog Acquisition and Updating}
%\subsection{List of Functions, Vendors, and Types}

 
%\anat{ y- ercentage of functions with  }

\label{sec:catalog_acquistion}
%\barm{first list, update vendor and then handle mistakes}

Through the previous section, we have been working with the assumption that we already have the necessary catalogs, vendor types, and functions for the sake of simplicity. This section explores systematic techniques to create and maintain the various catalogs. Our method involves automatically mining the Internet for information, beginning with mining the shorter and more stable catalog of functions, continuing with the long catalog of vendors, and concluding with the longest and most comprehensive catalog of types $T$. Then we discuss how we can update the list on the fly, and how we can deal with errors in the catalogs, such that the vendor or type are not in the catalog. We note that this was not our focus in the research, and more is left to future work. However, as we show the promising preliminary results, and a clear direction for a solution. 

\subsubsection{Catalog Acquisition}


As described, from Section  \ref{sec:dataset} we assembled a catalog of functions for IoT home devices,  based on information about IoT home devices from Fing \cite{Dev_Recogn_API_2019}, eCommerce sites \cite{amazon_search,ebay_search,ali_express}, and ChatGPT. This catalog is stable and new functions are rarely added. If an update is needed to this function catalog, we can update it manually.
 
In the second phase, we acquired the vendor catalog and type catalog. For each function $f \in F$ in the function catalog, we obtained vendors using again the above commercial sites, i.e., asking chatgpt what are the top IoT camera vendor and so on. For each vendor $v$ found, we added  $(v,f)$ to the $T$ type catalog of types. If the vendor $v$ was not already in $V$, we added it to $V$ as well. At the end of this process, our catalog contained 120 vendors and 278 types. Our dataset consists of 60 vendors and 100 types, i.e.,  %\anat{Need to give real details}.
The type and vendor catalog includes many more labels than what appears in the dataset. There were only 3 devices that were added to the catalog manually by us, i.e., the success of the technique was around $96\%$. However, we note the limitation in this experiment, since we use academic datasets, the devices are usually the common ones.  

\subsubsection{Vendor Catalog Update}
The vendor catalog needs to be updated as more players enter the market often. In this section, we present a technique to update the catalog using the traffic log of devices.

We used the GPT model to extract \textit{Named Entities} from the device trafic log. Named-entity recognition (NER) is an information extraction task that classifies entities mentioned in text into pre-defined categories such as person names, organizations, and etc.
Our method of updating this catalog consists of two distinct stages:
\begin{itemize}
    \item \textbf{Extract Vendor Entities from Data} - For NER model, we used GPT, which can be adapted to recognize named entities. For each device we used the enriched features of our dataset search results as input to the NER-Based-GPT model. To instruct the model, we provided a structured prompt directing it to identify and extract entities relevant to our context. The exact prompt used for this task is detailed in Appendix \ref{app:prompt}.
    \item \textbf{Entity Catalog Filter} - Post-extraction, we observed that the catalog of named entities contained entries not exclusively related to IoT vendors. To address this, we used GPT to validate each entity from the extracted catalog against a single criterion: its association with IoT manufacturing. The prompt we used for this phase is as follows: %\ref{app:prompt}). %Through this iterative validation, we were able to refine our catalog such that it included predominantly IoT and network device vendors. 
\end{itemize}

\begin{mdframed}[frametitle={GPT4, Prompt, Filter Entities}]
    "I will provide you a list of elements, extracted by a NER system. For each one of them check if they represent a name of an IoT manufacturer or another manufacture of Network devices and output it as a list of the elements and True/False flag"
\end{mdframed}
 %\anat{give statistics... how many of the functions you cover, how many of the vendors you cover ... and how many of the types you cover.. from the list.} %\barm{I added some, I'm not sure I really can put here information since we built it somehow differently}. 
%To validate our method, we examined our dataset device, we found that all of the vendors and functions appear in the eCommerce sites mentioned.  We leave to future work, ways to improve the techniques of obtaining the catalog.  Note that the procedure for acquiring these catalogs should be conducted on a regular basis to ensure their updates. Moreover, this process only involves the addition of new items, without the removal of existing ones from the catalogs.
%\subsection{Integration with the String Matching Algorithm}

To evaluate whether our catalog update achieved its goal, we experiment it. We run the algorithm with a catalog of vendors, that was extracted and then filtered using our method. The results are given in Table \ref{tab:vendor-experiments} in the row of the Acquired catalog. Interestingly, the results using our acquired catalog (0.76, HIT1) are comparable to those that used our generated vendor catalog (0.86, HIT1).

We should note that since new vendors can emerge over time, we recommend periodically running the vendor updating algorithm on all traffic logs. This allows us to check if the algorithm discovers a new vendor and, if so, whether the score of the new vendor exceeds that found by our IoT labeling algorithm. In such a case, we should update the vendor catalog and prioritize the new vendor as the label.
%Then we examined the properties of the list of types. 
\ignore{\begin{figure*}
     \centering
     \begin{subfigure}[h]{0.45\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/vendor_function_count.png}
                  %\vspace{-0.8cm}
\caption{}

\label{fig:device_types_cdf}
\end{subfigure}
     \begin{subfigure}[h]{0.45\linewidth}
         \centering
         \includegraphics[width=\linewidth,height=5.3cm]{figures/cdf_vendor_types_list.png}
         %\vspace{-0.6cm}
\caption{}

\label{fig:device_vendors_cdf}
\end{subfigure}
%\vspace{-0.3cm}
\caption{The characteristics of the IoT catalog type (a) amount of vendors per unique function (b) CDF which represents percentage of vendors manufacturing varying numbers of distinct functions.}
\label{fig:combined_cdf}
\end{figure*}
}
%Figure \ref{fig:combined_cdf} reveals that 75\% of the functions in the catalog have more than 5 vendors,  while 75\% of the vendor provide no more than two functions. These results reflect the nature of the IoT market, in which many companies focus on one or a few functions, yet several companies are competing within each function of IoT. An important implication of these findings is that accurately identifying the vendor, in most cases, would reveal the function or, at the very least, narrow it down to a few potential choices.

\subsubsection{Type Catalog Update}

Another scenario we need to cope is when a known vendor enters a new market and introduces a device function that it didn't have before. To address this situation, we recommend always cross-referencing against the complete functions catalog and comparing scoring results with the narrower catalog specific to the vendor. If a higher matching score is found in the complete catalog, we would then perform another check using ChatGPT to verify that the function is indeed provided by the manufacturer. If confirmed, the link update the type catalog accordingly.
